Elements of naturality in dynamical simulation frameworks for Hamiltonian, thermostatic, and Lindbladian flows on classical and quantum state-spaces

The practical focus of this work is the dynamical simulation of polarization transport processes in quantum spin microscopy and spectroscopy. The simulation framework is built-up progressively, beginning with state-spaces (configuration manifolds) that are geometrically natural, introducing coordinates that are algebraically natural; and finally specifying dynamical potentials that are physically natural; in each respect explicit criteria are given for "naturality." The resulting framework encompasses Hamiltonian flow (both classical and quantum), quantum Lindbladian processes, and classical thermostatic processes. Constructive validation and verification criteria are given for metric and symplectic flows on classical, quantum, and hybrid state-spaces, with particular emphasis to tensor network state-spaces. Both classical and quantum examples are presented, including dynamic nuclear polarization (DNP). A broad span of applications and challenges is discussed, ranging from the design and simulation of quantum spin microscopes to the design and simulation of quantum oracles.

==> QSE_JCP_defined_acronyms.tex <==

% ****************************************************************
% define acronym macros
% ****************************************************************
\RequirePackage{graphicx}
\RequirePackage{xspace} 

\newcommand{\mySmallMag}{0.953}
\newcommand{\mySmallBox}[2][\mySmallMag]{\protect\scalebox{#1}{\mbox{#2}}}
\newcommand{\myAcronym}[1]{\mySmallBox{#1}\xspace}
\newcommand{\myCodename}[1]{\mySmallBox[1.25]{\scshape #1}\xspace}
% ****************************************************************

% ****************************************************************
% acronyms definitions
% ****************************************************************
\newlength{\myKheight}
\newcommand{\mytextK}%
{%
	\settoheight{\myKheight}{K}%
	\resizebox{!}{1.03\myKheight}{\ensuremath{\lcal{K}}}%
}
\newcommand{\IBM}{\myAcronym{IBM}}
\newcommand{\UW}{\myAcronym{UW}}
\newcommand{\QSE}{\myAcronym{QSE}}
\newcommand{\SVD}{\myAcronym{SVD}}
\newcommand{\SAT}{\myAcronym{SAT}}
\newcommand{\NP}{\myAcronym{NP}}
\newcommand{\DNP}{\myAcronym{DNP}}
\newcommand{\USA}{\myAcronym{USA}}
\newcommand{\MPS}{\myAcronym{MPS}}
\newcommand{\KLISP}{\myAcronym{{\mytextK}LISP}}

\newcommand{\NOSQUISH}{\myCodename{no\hspace{-0.05em}\_\hspace{+0.05em}squish}}
\newcommand{\SIMPSON}{\myCodename{simpson}}
\newcommand{\SPINEVOLUTION}{\myCodename{spinevolution}}

% ****************************************************************





==> QSE_JCP_latex_macros.tex <==

% ****************************************************************
% optional font packages
% ****************************************************************
\RequirePackage{eucal}
% ****************************************************************

% \usepackage{caprule}


% ****************************************************************
% accented words
% ****************************************************************
\newcommand  {\Kahler}         {K\"{a}hler}
\newcommand  {\Kahlerian}      {K\"{a}hlerian}
\newcommand  {\Ito}            {It\^{o}}

\newcommand{\myTableOneEntry}[1]{\scalebox{0.925}{{\sffamily({\bfseries1#1})}}}
\newcommand{\myTableTwoEntry}[1]{\scalebox{0.925}{{\sffamily({\bfseries2#1})}}}
\newcommand{\myTableThreeEntry}[1]{\scalebox{0.925}{{\sffamily({\bfseries3#1})}}}
\newcommand{\myTableFourEntry}[1]{\scalebox{0.925}{{\sffamily({\bfseries4#1})}}}

% ****************************************************************

% ****************************************************************
% text words
% ****************************************************************
\newcommand{\HtwoO}{\ensuremath{\text{H}_2\text{O}}}


% ****************************************************************
% mathematical macros
% ****************************************************************

\newtheorem{theorem}{\mdseries\scshape Theorem}
\newtheorem{lemma}[theorem]{\mdseries\scshape Lemma}
\newtheorem{proposition}[theorem]{\mdseries\scshape Proposition}
\newtheorem{definition}[theorem]{\mdseries\scshape Definition}
\newtheorem{corollary}[theorem]{\mdseries\scshape Corollary}

\newtheorem*{resolution}{\mdseries\scshape Proposition}

\newtheorem{challenge}{\mdseries\scshape Challenge}

\definecolor{myChallengeColor}{rgb}{0.875,0.965,0.875}

\newcommand{\myChallengeBox}[2]{\vspace{0.5\baselineskip}{%
\small%
\setlength{\fboxsep}{0.45em}% customize the box separation
\setlength{\fboxrule}{1pt}% customize the box rule width
\noindent%
\hspace*{-0.333\fboxrule}% arrange for a very mild overhang
\makebox[\width+0.333\fboxrule][l]{%
\fcolorbox{black}{myChallengeColor}{\begin{minipage}{\columnwidth-2\fboxsep-2\fboxrule+0.666\fboxrule}%
\begin{challenge}[\scshape #1]%
\hspace*{-0.1em}\rule{0pt}{0pt}\vspace{0.3\baselineskip}\protect\newline\noindent%
#2%
\end{challenge}%
\end{minipage}}%
}}\vspace{0.5\baselineskip}}


\DeclareMathOperator{\mydim}{\text{dim}}
\DeclareMathOperator{\tr}{\text{tr}}
\DeclareMathOperator{\sgn}{\text{sgn}}
\DeclareMathOperator{\rank}{\text{(metric) rank}}
\DeclareMathOperator{\arctantwo}{\text{arctan}}
\DeclareMathOperator{\Image}{\text{Im}}
\DeclareMathOperator{\Kernel}{\text{Ker}}
\DeclareMathOperator{\Span}{\text{Span}}

\newcommand{\myscriptHermitian}{\text{\sffamily H}}

\newcommand{\dimH}{\ensuremath{\dim_{\hspace{0.1em}\mathbb{R}} \mathcal{H}}}
\newcommand{\scriptH}{\ensuremath{\mathcal{H}}}
\newcommand{\scriptK}{\ensuremath{\mathcal{K}}}
\newcommand{\mydIto}[1]{\mydelta\hspace{0.05em}#1}

% \RequirePackage{amsmath}
%	\RequirePackage{amssymb}
% \providecommand{\notag}{\nonumber}
\RequirePackage{bm}

\newcommand{\myEnsuremath}[1]{\ensuremath{#1}}  
% \newcommand{\myBoldsymbol}[1]{\boldsymbol{#1}}
\newcommand{\myBoldsymbol}[1]{\bm{#1}}
\newcommand{\myHat}[1]{\Hat{#1}}
\newcommand{\myBar}[1]{\Bar{#1}}


% For reference on the idioms used, see ...
% Command syntax:         Gratzner Section  9.1, pp 267-276.
% Math fonts:             Gratzner Section A.13, pp 355.
% Overstrikes and tildes: Gratzner Section A.12, pp 355.
% Delimiters:             Gratzner Section  4.6, pp 152.


\newcommand*{\myMathcal}[1]{\mathcal{#1}}
\newcommand*{\myMathfrak}[1]{\mathfrak{#1}}
\newcommand*{\myMathbb}[1]{\mathbb{#1}}
\newcommand*{\myMathbf}[1]{\mathbf{#1}}
\newcommand*{\myPrime}[1]{{#1'}} 
\newcommand*{\myPprime}[1]{{#1''}} 
\newcommand*{\myDot}[1]{{\dot{#1}}}
\newcommand*{\myDdot}[1]{{\ddot{#1}}}

% Adorning variables: mnemonic rules:
% "s" commands apply to symbols only
% "l" commands apply to latin characters
% "gs" commands apply to greek characters

% Symbols with accents
\newcommand*{\stilde}[1]{\myEnsuremath{\tilde{#1}}}
\newcommand*{\shat}[1]{\myEnsuremath{\myHat{#1}}}
\newcommand*{\svec}[1]{\myEnsuremath{\vec{#1}}}
\newcommand*{\sbar}[1]{\myEnsuremath{\myBar{#1}}}
\newcommand*{\sprime}[1]{\myEnsuremath{\myPrime{#1}}}
\newcommand*{\spprime}[1]{\myEnsuremath{\myPprime{#1}}}
\newcommand*{\sdot}[1]{\myEnsuremath{\myDot{#1}}}
\newcommand*{\sddot}[1]{\myEnsuremath{\myDdot{#1}}}

% Greek bold characters with accents (Latin characters disparaged)
\newcommand*{\gsb}[1]{\myEnsuremath{\myBoldsymbol{#1}}}
\newcommand*{\gsbtilde}[1]{\myEnsuremath{\tilde{\gsb{#1}}}}
\newcommand*{\gsbhat}[1]{\myHat{\gsb{#1}}}
\newcommand*{\gsbbar}[1]{\myBar{\gsb{#1}}}
\newcommand*{\gsbprime}[1]{\myPrime{\gsb{#1}}}
\newcommand*{\gsbpprime}[1]{\myPprime{\gsb{#1}}}
\newcommand*{\gsbdot}[1]{\myDot{\gsb{#1}}}
\newcommand*{\gsbddot}[1]{\myDdot{\gsb{#1}}}

% Latin bold characters with accents (Latin characters disparaged)
\newcommand*{\lb}[1]{\gsb{#1}}
\newcommand*{\lbtilde}[1]{\myEnsuremath{\tilde{\lb{#1}}}}
\newcommand*{\lbhat}[1]{\myHat{\lb{#1}}}
\newcommand*{\lbbar}[1]{\myBar{\lb{#1}}}
\newcommand*{\lbprime}[1]{\myPrime{\lb{#1}}}
\newcommand*{\lbpprime}[1]{\myPprime{\lb{#1}}}
\newcommand*{\lbdot}[1]{\myDot{\lb{#1}}}
\newcommand*{\lbddot}[1]{\myDdot{\lb{#1}}}

% Latin variant fonts (disparaged)
\newcommand*{\lcal}[1]{\myEnsuremath{\myMathcal{#1}}}
\newcommand*{\lbcal}[1]{\myEnsuremath{\gsb{\myMathcal{#1}}}}
\newcommand*{\lbb}[1]{\myEnsuremath{\myMathbb{#1}}}
\newcommand*{\lfrak}[1]{\myEnsuremath{\myMathfrak{#1}}}
\newcommand*{\lbfrak}[1]{\myEnsuremath{\gsb{\myMathfrak{#1}}}}

% Latin character typefaces
\newcommand*{\lsf}{\mathsf}%math sans serif
\newcommand*{\ltt}{\mathtt}%math typewriter

% text mode font shortcuts
\newcommand*{\tbf}{\textbf}%text bold
\newcommand*{\tit}{\textit}%text italic
\newcommand*{\tsl}{\textsl}%text slanted
\newcommand*{\tsc}{\textsc}%text small cap
\newcommand*{\ttt}{\texttt}%text typewriter
\newcommand*{\trm}{\textrm}%text roman
\newcommand*{\tsf}{\textsf}%text sans serif
\newcommand*{\tup}{\textup}%text upright

% Macros for Dirac bra-ket notation
\newcommand*{\braket}[3]{\myEnsuremath{\langle#1|#2|#3\rangle}}
\newcommand*{\inner}[2]{\myEnsuremath{\langle#1|#2\rangle}}
\newcommand*{\expect}[1]{\myEnsuremath{\langle#1\rangle}}
\newcommand*{\bra}[1]{\myEnsuremath{\langle#1|}}
\newcommand*{\ket}[1]{\myEnsuremath{|#1\rangle}}


\newsavebox{\mydeltaimage}
\savebox{\mydeltaimage}{%
\includegraphics{differentialDup.pdf}
}
\newlength{\mydeltadheight}
\newcommand{\mydelta}{\raisebox{0pt}[0pt][0pt]{%
\settoheight{\mydeltadheight}{\mbox{\ensuremath{d}}}%
\raisebox{0.00ex}{%
\resizebox{!}{\mydeltadheight}{\usebox{\mydeltaimage}}%
\hspace{0.05em}}%
}}%

\newcommand{\myequiv}% nicer \triangleq
{\ensuremath%
	{\mathbin%
		{\stackrel%
			{\makebox[\width][c]%
				{\protect\raisebox{-0.125ex}[0pt][0pt]%
			  	{\scalebox{0.80}[0.65]%
						{\scriptsize\sffamily def}}}}%
			{\hspace{0.1em}\raisebox{-0.125ex}[\height][0pt]{$=$}\hspace{0.1em}}}}}%


\newcommand{\myJstar}{%
	\makebox[\width][c]{%
		\raisebox{0pt}[\height][0pt]{%
			\ensuremath{J^{\hspace{-0.0em}\ast\hspace{-0.05em}}}}}}
				
\newcommand{\myJstarinv}{%
	\makebox[\width][c]{%
		\raisebox{0pt}[\height][0pt]{%
			\ensuremath{(\myJstar)^{\scriptstyle\hspace{+0.025em}\text{--1}}}}}}

\newcommand{\mycirc}{{\raisebox{0.15ex}{\scriptsize\ensuremath{\,\circ\,}}}}%

\newcommand{\myBundleMap}[3][\tilde]{%
	{#1{\hspace{-0.05em}\phi\hspace{0.05em}}}%
		_{\hspace{-0.1em}#2}%
		^{\raisebox{-0.4ex}{%
			\text{$\scriptstyle\hspace{0.1em}#3$}}}%
}
			


%	\newcommand{\myoverline}[1]{%
%	\overset{\smash{\ldots}}{#1}}

%	\newcommand{\myoverline}[1]{%
%	\overset{%
%	\hspace*{-0.05em}%
%	\scalebox{1.6}[1]{%
%		\rotatebox{90}{\tiny%
%			\raisebox{-0.5\height}[0pt][0pt]{%
%				\makebox[0pt][c]{\sffamily]}}}}
%	}{#1}}


% ****************************************************************



